Induced Distributions from Generalized Unfair Dice

In this paper we analyze the probability distributions associated with rolling (possibly unfair) dice infinitely often. Specifically, given a $q$-sided die, if $x_i\in\{0,\ldots,q-1\}$ denotes the outcome of the $i^{\text{th}}$ toss, then the distribution function is $F(x)=\mathbb{P}[X\leq x]$, where $X = \sum_{i=1}^\infty x_i q^{-i}$. We show that $F$ is singular and establish a piecewise linear, iterative construction for it. We investigate two ways of comparing $F$ to the fair distribution -- one using supremum norms and another using arclength. In the case of coin flips, we also address the case where each independent flip could come from a different distribution. In part, this work aims to address outstanding claims in the literature on Bernoulli schemes. The results herein are motivated by emerging needs, desires, and opportunities in computation to leverage physical stochasticity in microelectronic devices for random number generation.

==> zz_cut_material.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%~~~~~~~~~~~~~~~~ CUT OLD INTRO MATERIAL ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Decades of computer engineering have instilled determinism into every conceivable facet of computational computing. This is not without exceptional reason: we want our computational machines to function correctly and do so in an infallible manner. Stochastic behavior is often seen as contrary to such goals. As such, noise and fluctuations have been eliminated or constrained wherever possible.

%Deterministic computers, however, are nearing their limit with the end of Moore's Law and Dennard's Scaling. Extremely high-dimensional problems require reduced order models (through specialists or through artificial intelligence (AI)) or require particle method and probabilistic approaches. Even approaches utilizing AI can be probabilistic in nature, leveraging Bayesian learning techniques. For all of these probabilistic problems, and other uses of randomness like cryptography, we rely on pseudo-stochasticity added as software through pseudo-random number generators (pRNG).

%While pRNG has met needs for many applications, it is not without its failures. Of particular historical notoriety, the RANDU generator's iterates in three dimensions fall along planes \cite{markowsky2014sad}. As our needs for true randomness grow, we cannot help but ask why we do not solve probabilistic problems using true probabilistic computers?

%%The future of computing must embrace both heterogeneity and specialization. The end of Moore's law and Dennard's scaling along with growing needs for increasingly complicated computation with ever decreasing latency demands will naturally drive computation solutions towards highly heterogeneous computation with specialized components. \textbf{[CITE SOMETHING]}

%%Quantum computing has exploded with interest due to pressing problems in the field. Quantum problems are inherently probabilistic and complicated. Modern computational design expends time and energy to ensure that devices do not behave randomly and probabilistic factors are typically added after the fact as pseudo-random number generators (pRNG). These are not sufficient for many problems, including cryptography and certain quantum problems, and novel technology can produce major impact today while quantum computers are developed.

%The need for probabilistic computing and devices (and their uses) has grown in recent years and has been noted throughout the literature \cite{misra2022probabilistic,chowdhury2023accelerated,chowdhury2023full,aadit2022massively,kaiser2021probabilistic}. Answering this need, certain devices, such as magnetic tunnel junctions \cite{rehm2022stochastic,liu2022random} or tunnel diodes \cite{bernardo2017extracting}, can be made to behave as an effective Bernoulli random variable (hereafter, a coinflip). These devices have some probability $p$ of returning 1 and a probability $1-p$ of returning 0. While not glamorous, such simple random variables have great utility and can be exploited to return samples from a variety of distributions \cite{gryszka2021biased,flegal2012exact}. Furthermore, when used as input to novel and emerging hardware, like spiking neurons in a neuromorphic computer, such simple stochastic input can be sued to solve complicated NP-hard problems like MAXCUT \cite{theilman2022stochastic,theilman2023goemans}.

%While the roadmap for probabilistic computing efforts is to eventually compute directly on distribution in hardware, the first step is to utilize noisy devices like magnetic tunnel junctions and tunnel diodes to produce useful and efficient random numbers through effective coinflips.  It is worth noting that these devices could conceivably behave not as just coins, but as $n$-sided dice. Indeed, current devices considered for other purposes can be in one of five states \cite[Fig. 2e]{leonard2023stochastic}. Though the bulk of current investigations examine coin-like devices, such as the $p$-bits \cite{camsari2017stochastic}, in the future we may find that dice-like devices are more attractive for physical reasons (more stable or more efficient) or perhaps even for computational ones (reduced burden or circuitry).

%Nonetheless, with any hardware implementation of randomness, there will be uncertainty around behavior. It is conceivable that a given device may or may not behave as a fair coin or a truly fair die. Given that fair rolls or flips are needed to produce uniform random numbers, the basis of nearly all standard pRNG distributions, it is critical to understand departure from uniform in the general setting.

%Given the growing interest around probabilistic computing and the need to understand deviations from uniformity, we examine binary encoded distributions from Bernoulli coinflips and $n$-ary encoded distributions from $n$-sided die rolls. We revisit classic results in the Bernoulli case for a class of singular measures and extend these results to the $n$-sided die case, providing for each a distance from uniform for unfair cases.  These formula stand to provide the basis for error analysis in the future of probabilistic computing.

%We organize this effort as follows. In Section \ref{sec:bernoulli}, we define binary encoded distributions from Bernoulli coinflips and summarize existing results. Then, we ...


%%The reality is that devices are noisy and that if leveraged properly we could impact real probabilistic computation by providing true random number generation.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%~~~~~~~~~~~~~~~~ CUT SAMPLES TO NOTICE DEVIATION ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Expected Samples to Notice Uniform Deviation with a Fair Coin\label{sec:expectedsamples}}

In any device setting, it is not likely to have a truly fair coin. Rather a coin may be engineered to be close to fair. Given that we use an unfair coin with probability of heads $p_1$ and tails $p_0$, how many $b$-bit binary decimals can we draw before we notice that the set of samples is not likely uniformly distributed?

Empirically, such a question can be answered with a hypothesis test. One first gathers a collection of $b$-bit samples from a biased coin; then formulates the null hypothesis that the samples are uniformly distributed. A test statistic is calculated and depending on the chosen significance level of the test we can conclude to either accept or reject the null hypothesis.

However, given that we know we will be using a biased coin, we know that the samples are not uniformly distributed. It makes more sense to ask at what number of samples $N$, on average, for a fixed significance level will I notice that my samples are not uniform?  This is an analytic question that we can solve using probability.

We will address this by using a $\chi^2$ test.  The $\chi^2$ test is a comparison between frequencies of categorical variables. It is critical to note that since we are assuming a $b$-bit binary number generated from flips of a biased coin, there are a finite number ($2^b$) of outcomes and we may treat these as defacto categorical data. To compare to the uniform distribution, we must discretize the uniform distribution into $2^b$ bins and find the expected frequency of uniform draws appearing in those bins over $N$ independent draws.  In this way we can compare the frequencies of the $b$-bit biased coin draws to the expected frequencies of a uniform distribution.  Alternatively, we could make the comparison to the expected frequencies of a $b$-bit fair coin draws. In this case, these two are the same and each bin would have an expected frequency of $N/2^b$.  As the null hypothesis is that these two frequencies should be the same (that is, the biased coin produces uniform samples), the test statistic will follow a $\chi^2$ distribution and hence the $\chi^2$ test may be applied.  The $\chi^2$ test statistic is given as:
\[\chi^2_{ts}=\sum_{i=1}^{2^b}\frac{\left(\mathcal{O}_i-\mathcal{E}_i\right)^2}{\mathcal{E}_i},\]
where $\mathcal{O}_i$ is the number of observations of type $i$ and $\mathcal{E}_i$ is the expected number of observations of type $i$.  For $N$ draws, $\mathcal{E}_i=N/2^b$ and $\mathcal{O}_i$ is the histogram value for the $i^\text{th}$ value over the $N$ draws.

Given a desired significance level, one may calculate a critical value for the test $\chi^2_{crit}$.  If $\chi^2_{ts}<\chi^2_{crit}$, then we accept the null hypothesis.  One may think of the significance level as the point at which the probability of receiving the sampled data under the null hypothesis is so low that you are no longer willing to accept the null hypothesis.

We seek to characterize the distribution of the number of samples gathered where you fail the hypothesis test.  That is, where $\chi^2_{ts}=\chi^2_{crit}$.  By the central limit theorem, as the number of trials of the hypothesis test increases to infinity, the distribution of the average point of failure will be normally distributed.  Therefore, we will only calculate the first and second moments of $N$.

To that end, let $\left\{\tau_i\right\}=\left\{\tau_1,\tau_2,\ldots\right\}$ be a collection of independent and identically distributed random variables.  These are distributed as the binary output of $b$-flips of a biased coin. Let $N$ be the number for which the first $N$ $\tau_i$ fail the hypothesis test.  Let $x_j$ be the $j^{\text{th}}$ possible outcome for the random variables -- $x_1$ is $b$ zeros and $x_{2^b}$ is $b$ ones.  Let $n_j$ be the number of ones in $x_j$.  Then $\mathbb{P}\left[\tau_i=x_j\right]=p_1^{n_j}p_0^{b-n_j}$.

Given the first $N$ samples of $\left\{\tau_i\right\}$, let $H\left(x_j,\left\{\tau_i\right\},N\right)$ be the histogram value for outcome $x_j$.  We may write
\begin{equation}
    H\left(x_j,\left\{\tau_i\right\},N\right) = \sum_{\ell=1}^N\mathbf{1}_{x_j}\left(\tau_\ell\right),
\end{equation}
where $\mathbf{1}$ represents the indicator function.

To find expressions for $\mathbb{E}\left[N\right]$ and $\mathbb{E}\left[N^2\right]$, we will first prove a few lemmas concerning $H$.

\begin{lemma}
For the variables described above,
\[\mathbb{E}\left[H\left(x_j,\taus,N\right)\,\middle|\,N\right] = Np_1^{n_j}p_0^{b-n_j}.\]
\end{lemma}

\begin{proof}
The proof proceeds by induction on $N$. For $N=1$, note
\begin{align*}
    \mathbb{E}\left[H\left(x_j,\taus,N\right)\,\middle|\,N=1\right] &= \mathbb{E}\left[\indi{x_j}{\tau_1}\right]\\
    &=\sum_{k=1}^{2^b}\indi{x_j}{x_k}\mathbb{P}\left[\tau_1=x_k\right]\\
    &=p_1^{n_j}p_0^{b-n_j}.
\end{align*}
Assume the result holds up to $N-1$. Then,
\begin{align*}
    \mathbb{E}\left[H\left(x_j,\taus,N\right)\,\middle|\,N\right] &= \mathbb{E}\left[\indi{x_j}{\tau_N} + \sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right]\\
    &=\mathbb{E}\left[\indi{x_j}{\tau_N}\right]+(N-1)p_1^{n_j}p_0^{b-n_j}\\
    &=Np_1^{n_j}p_0^{b-n_j}.
\end{align*}
\end{proof}

\begin{lemma}
    For the variables described above,
    \[\mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^2\,\middle|\,N\right]=Np_1^{n_j}p_0^{b-n_j} + N(N-1)\left(p_1^{n_j}p_0^{b-n_j}\right)^2\]
\end{lemma}

\begin{proof}
    Again the proof proceeds by induction on $N$.  For $N=1$, note
    \begin{align*}
        \mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^2\,\middle|\,N=1\right] &= \mathbb{E}\left[\left(\indi{x_j}{\tau_1}\right)^2\right]\\
        & = \sum_{k=1}^{2^b}\left(\indi{x_j}{x_k}\right)^2\mathbb{P}\left[\tau_1=x_k\right]\\
        &=p_1^{n_j}p_0^{b-n_j}.
    \end{align*}
    Assume the result holds up to $N-1$. Note that since $\tau_N$ is independent from all other $\tau_i$, that a function of $\tau_N$ will be independent from a function of all other $\tau_i$.  Then,
    \begin{align*}
        \mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^2\,\middle|\,N\right] &= \mathbb{E}\left[\left(\indi{x_j}{\tau_N}+\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right)^2\right]\\
        & = \mathbb{E}\left[\left(\indi{x_j}{\tau_N}\right)^2\right] + 2\mathbb{E}\left[\indi{x_j}{\tau_N}\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right] + \mathbb{E}\left[\left(\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right)^2\right]\\
        &=p_1^{n_j}p_0^{b-n_j} + 2\mathbb{E}\left[\indi{x_j}{\tau_N}\right]\mathbb{E}\left[\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right] \\
        &\qquad\qquad + (N-1)p_1^{n_j}p_0^{b-n_j} + (N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^2\\
        &=Np_1^{n_j}p_0^{b-n_j} + 2(N-1)\left(p_1^{n_j}p_0^{b-n_j}\right)^2 + (N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^2\\
        & = Np_1^{n_j}p_0^{b-n_j} + N(N-1)\left(p_1^{n_j}p_0^{b-n_j}\right)^2.
    \end{align*}
\end{proof}

With these two lemmas, we can find an expression for the expected value of $N$.

\begin{theorem}
    For the variables described above,
    \[\mathbb{E}\left[N\right] = \frac{\chi^2_{crit} + 2^b\sum_{j=0}^b\binom{b}{j}\left(p_1^jp_0^{b-j}-\frac{1}{2}\right)^2-\frac{2^{2b}}{4}}{2^b\sum_{j=0}^b\binom{b}{j}\left(p_1^jp_0^{b-j}-\frac{1}{2^b}\right)^2}\]
\end{theorem}

\begin{proof}
    First, note that $N$ must be non-zero. In order to fail the hypothesis test, there must have been some evidence taken to conduct the hypothesis test. Next, note that $\mathbb{E}[N]$ must be finite. We have assumed we have a biased coin. We have previously shown that biased coins do not produce the uniform distribution. Therefore as more samples are drawn, the differences in expected frequencies will become more apparent until the hypothesis test is failed. Ergo, the expected value of any bin of the histogram of resulting samples must be finite too.  Hence, we may write
    \begin{align*}
        \mathbb{E}\left[\frac{\left(H\left(x_j,\taus,N\right)-N/2^b\right)^2}{N/2^b}\right]&=\mathbb{E}\left[\mathbb{E}\left[\frac{\left(H\left(x_j,\taus,N\right)-N/2^b\right)^2}{N/2^b}\,\middle|\,N\right]\right]\\
        &=\mathbb{E}\left[\frac{2^b}{N}\mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^2\,\middle|\,N\right]-2\mathbb{E}\left[H\left(x_j,\taus,N\right)\,\middle|\,N\right]+\frac{N}{2^b}\right]\\
        &=2^b\left(p_1^{n_j}p_0^{b-n_j}-\frac{1}{2^b}\right)^2\mathbb{E}\left[N\right]-2^b\left(p_1^{n_j}p_0^{b-n_j}-\frac{1}{2}\right)^2 + \frac{2^b}{4}.
    \end{align*}

    Taking the expectation of the $\chi^2$ test statistic at the critical value yields
    \begin{align*}
        \chi^2_{crit} & = \mathbb{E}\left[\sum_{j=1}^{2^b}\frac{\left(H\left(x_j,\taus,N\right)-N/2^b\right)^2}{N/2^b}\right]\\
        &=2^b\mathbb{E}\left[N\right]\sum_{j=1}^{2^b}\left(p_1^{n_j}p_0^{b-n_j}-\frac{1}{2^b}\right)^2 - 2^b\sum_{j=1}^{2^b}\left(p_1^{n_j}p_0^{b-n_j}-\frac{1}{2}\right)^2 + \frac{2^{2b}}{4}.
    \end{align*}

    Now, we note that $j$ only appears in the $n_j$ term which describes the number of ones appearing in the binary decimal $x_j$. Multiple binary decimals have the same number of ones. We recast these sums by summing over binary decimals having $j$ ones:
    \[\chi^2_{crit}=2^b\mathbb{E}\left[N\right]\sum_{j=0}^{b}\binom{b}{j}\left(p_1^{j}p_0^{b-j}-\frac{1}{2^b}\right)^2 - 2^b\sum_{j=0}^{b}\binom{b}{j}\left(p_1^{j}p_0^{b-j}-\frac{1}{2}\right)^2 + \frac{2^{2b}}{4}.\]
    Solving for $\mathbb{E}\left[N\right]$ proves the result.
\end{proof}

Obtaining the variance of $N$ is a little trickier.  We will find by taking the expected value of the square of the test statistic when it equals the critical value:
\begin{align*}
    \left(\chi^2_{crit}\right)^2 &= \left(\sum_{j=1}^{2^b}\frac{\left(H\left(x_j,\taus,N\right)-N/2^b\right)^2}{N/2^b}\right)^2\\
    &= \sum_{j=1}^{2^b}\frac{\left(H\left(x_j,\taus,N\right)-N/2^b\right)^4}{N^2/2^{2b}} + \sum_{j=1}^{2^b}\sum_{k\neq j}\frac{\left(H\left(x_j,\taus,N\right)-N/2^b\right)\left(H\left(x_k,\taus,N\right)-N/2^b\right)}{N^2/2^{2b}}.
\end{align*}

The first term on the left-hand side can be addressed in a similar manner to the previous, requiring only two more moments of $H$ given $N$. The second term is more challenging and will require another lemma in its own right.


\begin{lemma}
    For the variables described above,
    \[\mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^3\,\middle|\,N\right]=Np_1^{n_j}p_0^{b-n_j}+3N(N-1)\left(p_1^{n_j}p_0^{b-n_j}\right)^2 + N(N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^3.\]
\end{lemma}

\begin{proof}
    The proof proceeds by induction on $N$. For $N=1$:
    \begin{align*}
        \mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^3\,\middle|\,N=1\right] &= \mathbb{E}\left[\left(\indi{x_j}{\tau_1}\right)^3\right]\\
        & = \sum_{k=1}^{2^b}\left(\indi{x_j}{x_k}\right)^3\mathbb{P}\left[\tau_1=x_k\right]\\
        &=p_1^{n_j}p_0^{b-n_j}.
    \end{align*}
    Assume the result holds up to $N-1$. Then, from independence of the $\tau_i$,
    \begin{align*}
        \mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^3\,\middle|\,N\right]&= \mathbb{E}\left[\left(\indi{x_j}{\tau_N}+\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right)^3\right]\\
        &=\mathbb{E}\left[\left(\indi{x_j}{\tau_N}\right)^3\right]+3\mathbb{E}\left[\left(\indi{x_j}{\tau_N}\right)^2\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right] \\
        &\qquad\qquad + 3\mathbb{E}\left[\indi{x_j}{\tau_N}\left(\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right)^2\right] + \mathbb{E}\left[\left(\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right)^3\right]\\
        &=p_1^{n_j}p_0^{b-n_j} + 3\mathbb{E}\left[\left(\indi{x_j}{\tau_N}\right)^3\right]\mathbb{E}\left[\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right]\\
        &\qquad\qquad + 3\mathbb{E}\left[\indi{x_j}{\tau_N}\right]\mathbb{E}\left[\left(\sum_{\ell=1}^{N-1}\indi{x_j}{\tau_\ell}\right)^2\right] + (N-1)p_1^{n_j}p_0^{b-n_j}\\
        &\qquad\qquad + 3(N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^2\\
        &\qquad\qquad+ (N-1)(N-2)(N-3)\left(p_1^{n_j}p_0^{b-n_j}\right)^3.\\
        &=Np_1^{n_j}p_0^{b-n_j} +3p_1^{n_j}p_0^{b-n_j}\left((N-1)p_1^{n_j}p_0^{b-n_j}\right)\\
        &\qquad\qquad +3p_1^{n_j}p_0^{b-n_j}\left((N-1)p_1^{n_j}p_0^{b-n_j} + (N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^2\right)\\
        &\qquad\qquad + 3(N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^2\\
        &\qquad\qquad+ (N-1)(N-2)(N-3)\left(p_1^{n_j}p_0^{b-n_j}\right)^3.\\
        &=Np_1^{n_j}p_0^{b-n_j}+3N(N-1)\left(p_1^{n_j}p_0^{b-n_j}\right)^2 + N(N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^3.
    \end{align*}
\end{proof}

\begin{lemma}
    For the variables described above,
    \begin{align*}
        \mathbb{E}\left[\left(H\left(x_j,\taus,N\right)\right)^4\,\middle|\,N\right]&= Np_1^{n_j}p_0^{b-n_j} + 7N(N-1)\left(p_1^{n_j}p_0^{b-n_j}\right)^2+ 6N(N-1)(N-2)\left(p_1^{n_j}p_0^{b-n_j}\right)^3\\
        &\qquad\qquad+ N(N-1)(N-2)(N-3)\left(p_1^{n_j}p_0^{b-n_j}\right)^4.
    \end{align*}
\end{lemma}

As it involves induction as well as the same tricks and algebra as the previous three lemmas, we omit this proof.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ CUT TIKZ FIGURES ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
    \begin{tikzpicture}[ultra thick,scale=1]
				\begin{axis}[ axis lines=middle,
					clip=false,
					ymin=-0.5,
					ymax=1.5,
					xmin=-0.5,
					xmax=1.5,
					ytick={0,1},
		        	xtick={-1,0,1}
					]
					\addplot[very thick,color=cyan, domain=0:1]{1};
					\addplot[very thick,<-,color=cyan, domain=-0.5:0]{0};
					\addplot[very thick,->,color=cyan, domain=1:1.5]{0};
					\addplot[mark=o,color=cyan,mark size=3pt] coordinates {(0,0)};
					\addplot[mark=o,color=cyan,mark size=3pt] coordinates {(1,0)};
					\addplot[mark=*,color=cyan,mark size=3pt] coordinates {(0,1)};
					\addplot[mark=*,color=cyan,mark size=3pt] coordinates {(1,1)};
				\end{axis}
			\end{tikzpicture} 
			\caption{PDF for a fair coin}
			\label{fig:pdffair}
			\end{center}
\end{figure}

\begin{figure}
\begin{center}
    \begin{tikzpicture}[ultra thick,scale=1]
				\begin{axis}[ axis lines=middle,
					clip=false,
					ymin=-0.5,
					ymax=1.5,
					xmin=-0.5,
					xmax=1.5,
					ytick={0,1},
		        	xtick={-1,0,1}
					]
					\addplot[very thick,color=cyan, domain=0:1]{x};
					\addplot[very thick,<-,color=cyan, domain=-0.5:0]{0};
					\addplot[very thick,->,color=cyan, domain=1:1.5]{1};
				\end{axis}
			\end{tikzpicture} 
			\caption{CDF for a fair coin}
			\label{fig:cdffair}
			\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ CUT COMMENTS FROM BERNOULLI SECTION ~~~~~~~~~~~~~~~~~~~~~~~~~%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\color{ForestGreen}
%\begin{conjecture}
%A pdf may be sampled using binary encoded coinflips $X_i\sim\text{Bernouli}\left(p_i\right)$ if and only if there exist constants $K_i$ such that for all $k=0,\ldots,2^{i-1}-2$ and for all $i\in\mathbb{N}\cup\{0\}$
%\[\frac{\mathbb{P}\left(\left(\frac{2k}{2^i},\frac{2k+1}{2^i}\right)\right)}{\mathbb{P}\left(\left(\frac{2k}{2^i},\frac{2k+2}{2^i}\right)\right)}=K_i.\]
%In this case, necessarily $K_i=1-p_i$ and $p_i\to0.5$.
%\end{conjecture}
%Comments on this conjecture: In any binary encoded coinflip sampling, the first flip always determines the ratio of mass on either side of $0.5$.  The second flip proportions out each of the masses on $(0,0.5)$ and $(0.5,1)$ according to $p_2$ to fall on either side of $0.25$ and $0.75$ respectively.  This continues ad infinitum.  If we do not limit to $0.5$, then in the limit there is always mass to separate and dole out proportionally. However, if we do limit to $0.5$, then in the limit we no longer need to separate out and divide mass proportionally. We merely keep equal amounts on each side. In effect, this is a smoothness requirement.  We must tend to a point where differences in endpoints of dyadic intervals stop being too far apart.  Perhaps this relates to cdf or pdf conditions.

%The forward direction should be obvious.  If you have a pdf that can be sampled with coins, merely demonstrate that the ratio holds.  On the other hand, care would need to be taken in showing that a pdf with this ratio property could indeed be sampled by coins with $p_i=1-K_i$. Proving that $0.5$ is the limit would require the limit from conjecture 2 in conjunction.  In that if we have a distribution that can be sampled, then we must have this property otherwise the pdf would be zero.
%}\mycomment[jds]{Perhaps the 0.5 is a chunk too far.  But I stand by the other parts of this conjecture.}



%Theorem \ref{qsideddietheorem} is addressed in Section \ref{section:qsideddie}. Note that $q$ need not be prime. We only need $q\geq 2$ to guarantee that an arbitrary $X\in [0,1]$ has a $q$-adic expansion. This can be seen by considering the following classical result:

%\begin{theorem}[Theorem 7.11 in \cite{analysis1}]
%Suppose that $g\geq 2$. Then every real number $x$ has a base $g$ expansion. This expansion is unique if expansions satisfying $x_k=g-1$ for almost all $k\in \mathbb{N}$ are excluded. Moreover, $x$ is a rational number if and only if its base $g$ expansion is periodic.
%\end{theorem}
%\mycomment[dtp]{I suppose, then, it is more appropriate to write '$q$-ary' and not $q$-adic?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ CUT PROPOSITION FROM BERNOULLI SECTION ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Of note is that $p_0=0.24<0.5$ and the graph lies \textit{below} the cumulative distribution function for the uniform distribution \eqref{eq:uniform}. This observation is readily extended to a simple result. %This discussion motivates a few conjectures, discussions, and theorems:

\begin{proposition}
Let $F(x)$ (Eq. \ref{unfairrecursive}) be the CDF obtained from a binary encoding on i.i.d. Bernoulli flips as in \cite[Ex. 31.1]{billingsley}. For $x\in(0,1)$, if $p_0<1/2$, then $F(x)<x$ and if $p_0>1/2$, then $F(x)>x$. That is, the cumulative distribution function given in \eqref{eq:uniform} for the fair coin serves as a bounding function for the unfair cases.
\end{proposition}
\begin{proof}
    The proof is analogous for both $p<1/2$ and $p>1/2$. We shall demonstrate for $p<1/2$.

    Assume $p<1/2$ and suppose by way of contradiction that there exists an $\widehat{x}\in(0,1)$ such that $F\left(\widehat{x}\right)\geq\widehat{x}$.  First note that for any $2$-adic number $a\in(0,1)$ that $F(a)<a$.  Hence, in the case where $F\left(\widehat{x}\right)>\widehat{x}$ one need only choose an $a\in\left(\widehat{x},F\left(\widehat{x}\right)\right)$.  This violates the strictly increasing property of $F$ and hence no such $\widehat{x}$ can exist.

    If, however, $F\left(\widehat{x}\right)=\widehat{x}$, we must obtain a contradiction in cases.  Suppose $\widehat{x}\leq1/2$. 

    And ... I have no idea how to get a contradiction. Everything I do is broken.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ COMMENTS AND MATERIAL MOVED FROM MAIN DICE SECTION ~~~~~~~~~~~~~~~~~~~~~~~~~%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\mycomment[jds]{Thought more about this: If the pdf were infinite somewhere, then either $F$ would be improper, or (if dirac) would have a jump discontinuity. Since $\mathbb{P}(X=x)=0$ for all $x$, these cases do not happen and $F$ is continuous everywhere.}















The following is the old, broken proof of our main theorem:

\begin{theorem}\label{maintheorem2}
Consider a $q$-sided die, where $x_i\in\{0,\ldots,q-1\}$ denotes the outcome of the $i^\text{th}$ toss and $p_j:=\mathbb{P}[x_i=j]$ for $j\in\{0,\ldots,q-1\}$. Given $X = \sum_{i=1}^\infty x_iq^{-i}$, if $F(x)=\mathbb{P}[X\leq x]$ is the cumulative distribution function obtained after tossing the die an infinite number of times, then
\begin{enumerate}[(i)]
    \item If $p_j= \textstyle \frac{1}{q}$ for all $j$, then $F(x)=x$ on $[0,1]$ and \label{maintheorem2item1}
    \item If $p_j\neq \textstyle \frac{1}{q}$ for some $j$, then $F$ is singular.\label{maintheorem2item2}
\end{enumerate}
In either case, $F$ is given by the following recursion formula:
    \begin{equation} \label{qsideddierecursion}
    F(x) = 
    \begin{cases} 
    p_0F(qx) &\text{if} \ 0\leq x \leq \textstyle \frac{1}{q}\\
    p_0+p_1F(qx-1) &\text{if} \ \textstyle \frac{1}{q} \leq x \leq \frac{2}{q}\\
    \ \ \ \ \ \ \ \ \vdots &\ \ \ \ \ \ \ \ \ \vdots\\
    (p_0+p_1+\ldots+p_{q-2}) + p_{q-1}F(qx-(q-1)) &\text{if} \ \textstyle \frac{q-1}{q} \leq x \leq 1\\
    \end{cases}.
    \end{equation}
\end{theorem}
\begin{proof}
While (\ref{maintheorem2item1}) will follow from the recursion formula we will establish independently, we can also use the setting detailed in \eqref{eq:interval} to observe that, if $p_j=\textstyle \frac{1}{q}$ for all $j$, then
\[
F\left( \frac{k}{q^n}+\frac{1}{q^n}\right) - F\left( \frac{k}{q^n}\right) = F\left( \frac{k+1}{q^n}\right) - F\left( \frac{k}{q^n}\right) = p_{u_1}\cdot\ldots\cdot p_{u_n} = \frac{1}{q^n},
\]
which, due to the density of base-$q$ expansions in $[0,1]$, shows that $F(x)=x$.

We now establish (\ref{maintheorem2item2}). Take $X\in(0,1]$ and let $d_1(X), d_2(X),\ldots$ be the digits in its non-terminating base-$q$ expansion. If $\mu$ represents our probability measure, then $\mu[X\colon d_i(x)=j]=p_j$ for $j\in\{0,\ldots,q-1\}$. Consider
\begin{equation} \label{eq:sset}
S:=\left\{ x\in (0,1] \colon \lim_{n\to \infty} \frac{d_1(x)+\ldots+d_n(x)}{n} = p_0\cdot 0 + p_1\cdot 1 + \ldots + p_{q-1}\cdot (q-1) \right\}.
\end{equation}
For an $x$ sampled from the distribution of $X$, the strong law of large numbers implies that the average of the outcomes $d_i(x)$ tend toward the expectation $E(X) = p_0\cdot 0 + p_1\cdot 1 + \ldots + p_{q-1}\cdot (q-1)$ with probability 1 and therefore $\mu(S)=1$.

 On the other hand, %if we let $\#_x(a,n)=\#(a,n)$ denote the number of times $a\in \{0,\ldots,q-1\}$ appears in the first $n$ digits of the base-$q$ expansion for $x$, then 
 the normal number theorem guarantees that for almost every $x\in[0,1]$,%\mycomment[wms]{I think \# doesn't need to be redefined}
 \begin{align*}
     \lim_{n\to \infty} \frac{d_1(x)+\ldots+d_n(x)}{n} &= \lim_{n\to \infty} \frac{\#(0,n)\cdot 0 + \#(1,n)\cdot 1 +\ldots+ \#(q-1,n)\cdot (q-1)}{n}\\
     &= \lim_{n\to \infty} \frac{\#(0,n)}{n}\cdot 0+\frac{\#(1,n)}{n}\cdot 1+\ldots + \frac{\#(q-1,n)}{n}\cdot (q-1) \\
     &= \frac{1}{q}\cdot 0+\frac{1}{q}\cdot 1+\ldots + \frac{1}{q}\cdot (q-1).
 \end{align*}%\mycomment[wms]{I might be tired but why are these 1/3?
 
% Doug: This is the normal number theorem (see discussion at the top of page 6.
% William: Right, but why 1/3 specifically and not 1/q? (jds: they should be $1/q$, i'm betting it was a copypasta error. dtp: Yep. just a copy/paste error. My original proof was a 3-sided die proof and I was extending it to $q$-sided. I'll fix this.)
% }
Specifically, if
\begin{equation} \label{eq:tset}
T := \left\{  x\in(0,1]\colon   \lim_{n\to\infty}  \frac{d_1(x)+\ldots+d_n(x)}{n} =  \frac{1}{q}\cdot 0+\frac{1}{q}\cdot 1+\ldots + \frac{1}{q}\cdot (q-1)  \right\},
\end{equation}
then $\lambda(T)=1$, where $\lambda$ is Lebesgue measure on $[0,1]$.

Without loss of generality, assume $p_0 \neq \textstyle \frac{1}{q}$ and consider the sets
\[
S_0:= \left\{ x\in (0,1]\colon \lim_{n\to\infty} \frac{\#(0,n)}{n} = p_0 \right\} \hspace{.25in} \text{and} \hspace{.25in} T_0:=\left\{ x\in (0,1]\colon \lim_{n\to\infty} \frac{\#(0,n)}{n} = \frac{1}{q} \right\}.
\]
We see that $S\subseteq S_0 \subseteq [0,1]$.


\textcolor{blue}{How about this: For every $j$, form
\[
S_j:= \left\{ x\in (0,1]\colon \lim_{n\to\infty} \frac{\#(j,n)}{n} = p_j \right\},
\]
and consider
\[
\widetilde{S}:=\bigcap_{j=0}^n S_j.
\]
\textit{Borel's law of large numbers} says that, with probability 1, the frequency at which outcome $j$ occurs in the first $n$ trials tends toward $p_j$ as $n\to\infty$. That is, $\mu(S_j)=1$ for every $j$. Thus, by subadditivty of the measure $\mu$,
\[
\mu((\widetilde{S})^c) = \mu\left( \bigcup_{j=0}^n S_j^c \right) \leq \sum_{j=0}^n \mu(S_j^c) = 0,
\]
and therefore $\mu(\widetilde{S})=1$. Defined analogously, there are sets $T_j$ for which, when $\widetilde{T}:= \bigcap_{j=0}^n T_j$, we have $\lambda(T)=1$.}

\textcolor{blue}{Suppose there exists $p_k\neq \frac{1}{q}$. Then, by the uniqueness of limits, $S_k\cap T_k=\emptyset$, and therefore $\widetilde{S}\cap\widetilde{T}=\emptyset$. Thus, $\widetilde{S}$ and $\widetilde{T}$ are two disjoint sets with full measure for $\mu$ and $\lambda$, respectively. This implies that the two measures are mutually singular.}

%\textcolor{blue}{William, you've made a great point here. I think you are highlighting the same thing Darby has been highlighting recently: these sets $S$ and $T$ are not minimal. Your example shows that $S\not\subseteq S_0$, but also $S_0\not\subseteq S$, so this is not a `useful' set. When $q>2$, I can also fabricate a specific set of unfair probabilities that forces $S=T$, so not only will using these sets directly not work, but any proposed supersets of them won't be disjoint.}

%\textcolor{blue}{Thus, I think we really need to narrow down the set $S$ to a subset that better represents the support. Maybe, with
%\[
%S_j:= \left\{ x\in (0,1]\colon \lim_{n\to\infty} \frac{\#(j,n)}{n} = p_j \right\},
%\]
%we consider
%\[
%\widetilde{S}:=\bigcap_{j=0}^n S_j.
%\]
%In this case, we have $\widetilde{S} \subseteq S$. In fact, it would be proper I think. Moreover, since the Normal Number Theorem works term-by-term, the analogous sets for $T$ would have $\widetilde{T}=T$ and therefore $\lambda(\widetilde{T})=1$. Additionally, if we assume, without loss of generality, that $p_k \neq \frac{1}{q}$ for some $k$, then immediately $\widetilde{S}\cap \widetilde{T} = \emptyset$.}

%\textcolor{blue}{For this to work, I need to show $\mu(\widetilde{S})=1$, but I haven't gotten that far. Maybe there is a local interpretation of the Law of Large Numbers that works like the NNT does? Something that says ``with probability 1, the frequency of outcome $j$ tends toward $p_j$ for every $j$". Then $\mu(S_j)=1$ for all $j$ and hence $\mu(\widetilde{S})=1$.}

%\textcolor{blue}{These are just my thoughts. Maybe this is a bad idea for some obvious reason.
%}



\mycomment[wms]{Sorry I'm being dense, but is this true?  What about $111\ldots$ for $q=4$, $p_0=p_1=p_2=1/3$?} This concludes that $\mu(S_0)=1$ and so $\mu([0,1]\setminus S_0)=0$. Similarly, $T\subseteq T_0 \subseteq [0,1]$ and therefore $1=\lambda(T)\leq \lambda(T_0)\leq \lambda([0,1])=1$. This concludes that $\lambda(T_0)=1$ and so $\lambda([0,1]\setminus T_0)=0$. Finally, combining the assumption that $p_0\neq \textstyle \frac{1}{q}$ with the uniqueness of limits, we see that $S_0\cap T_0=\emptyset$. Thus, by Definition \ref{def:disjointsupp}, $\mu$ and $\lambda$ have disjoint supports. It now follows from Proposition \ref{prop:disjointsupports} that $F'(x)=0$ except on a set of Lebesgue measure 0 and therefore $F$ is singular.

 Finally, we establish the recursion formula given in (\ref{qsideddierecursion}). Note that $[0,1]$ can be divided into $q$ intervals $[0, \textstyle \frac{1}{q}], [\textstyle \frac{1}{q}, \frac{2}{q}],\ldots, [\textstyle \frac{q-1}{q},1]$ -- the so-called base-$q$ intervals of rank 1. We provide an explicit proof of the last case of the recursion formula since the previous cases follow similarly.

Suppose $x\in [\textstyle \frac{q-1}{q},1]$, the $q^\text{th}$ base-$q$ interval of rank 1. Here, $X \leq x$ can occur in $q$ different ways. Specifically, either $X$ lies in one of the previous base-$q$ intervals, or it lies in the last interval with $x$. Thus,
\begin{align*}
    \mathbb{P}[X \leq x] &= \mathbb{P}\left[ x_1=0 \ \text{or} \  \ldots \ \text{or} \ x_{1}=q-2 \ \text{or} \  \left(x_1=q-1 \ \text{and} \ \frac{q-1}{q} + \sum_{i=2}^\infty \frac{x_i}{q^i} \leq x\right)\right]\\
    &= (p_0 + \ldots + p_{q-2}) + p_{q-1}\mathbb{P}\left[q-1 + \sum_{i=2}^\infty \frac{x_i}{q^{i-1}} \leq qx\right]\\
    &= (p_0 + \ldots + p_{q-2}) + p_{q-1}\mathbb{P}\left[\sum_{i=1}^\infty \frac{x_{i+1}}{q^{i}} \leq qx-(q-1)\right]\\
    &= (p_0 + \ldots + p_{q-2}) + p_{q-1}\mathbb{P}\left[X \leq qx-(q-1)\right]\\
    &= (p_0 + \ldots + p_{q-2}) + p_{q-1}F(qx-(q-1)).
\end{align*}
Therefore, when $x\in [\textstyle \frac{q-1}{q},1]$, we have the recursion 
\[
F(x) = (p_0 + \ldots + p_{q-2}) + p_{q-1}F(qx-(q-1)).
\]
The rest of the cases follow similarly.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ~~~~~~ CUT FROM MAIN DICE SECTION ON 9/11/23 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{corollary} \label{corrolarrytomaintheorem1}
%    Given any $q$-sided die, there is only one choice of probabilities $p_j$ for which the associated probability measure $\mu$ is absolutely continuous relative to Lebesgue measure $\lambda$ and that is the one where all $j\in\{0,\ldots,q-1\}$ are equally likely. In this case, $\mu=\lambda$ almost everywhere on $[0,1]$.
%\end{corollary}
%\begin{proof}
%    We've shown that when $p_j\neq \textstyle \frac{1}{q}$ for some $j$, $\mu$ is singular with respect to Lebesgue measure. This leaves only the case where $p_j=\textstyle \frac{1}{q}$ for all $j$. In this case, we see that the sets $S$ and $T$ given in (\ref{eq:sset}) and (\ref{eq:tset}), respectively, are equal. Therefore, $\mu$ and $\lambda$ both have this common set as their supports, making $\mu=\lambda$ on $[0,1]$. \mycomment[dtp]{Is this proof sufficient?}
%\end{proof}

%\textcolor{red}{In the intro, simply note that uniform on $[0,1]$ is the same as Lebesgue restricted to $[0,1]$, so the future reference will hold as a result of the previous theorem.}

%\begin{remark}
%The bulk of the results in Theorems \ref{maintheorem1} and \ref{maintheorem2} serve to answer the questions posed in Problem 31.1 in \cite{billingsley}.
%\end{remark}

%    \item If $q\neq \widetilde{q}$ and either at least one of the two dice are unfair, then the associated probability measures, $\mu$ and $d\widetilde{\mu}$, are mutually singular.\mycomment[jds]{Why switch to $\mu$?}  \label{twodice2}

%https://math.stackexchange.com/questions/3720009/clarification-on-mutual-singularity-of-probability-measures

%For a finite word $w = w_1 w_2 \ldots w_n$, denote its cylinder set formed by all sequences starting with $w$ as $[w] = [w_1 w_2 \ldots w_n]$. \mycomment[wms]{I just wanted to get some notes down on what we talked about in the meeting about flat portions of the CDF. If it remains, it probably needs to be moved.}
%\begin{remark}
%The CDF is constant on some non-empty interval $[a,b]$, i.e.~$F(a) = F(b)$ for some $a < b$, if and only if there exists a $j$ such that $p_j = 0$.

%To see this, first we note that the following:
%\begin{enumerate}
%\item If $\mathbb{P}[X^\infty \in [w]] = 0$, then there exists some $j$ appearing in $w$ such that $\mathbb{P}[X^\infty \in [j]] = 0$ and, hence, $p_j = 0$.
%\item Likewise, if $p_j = 0$, then $\mathbb{P}[X^\infty \in [j]] = 0$ and $\mathbb{P}[X^\infty \in [w]] = 0$ for all $w$ containing $j$.
%\end{enumerate}

%The case where $p_j = 0$ follows directly from above setting $a = j/q$ and $b = (j+1)/q$.

%Assume that $a < b$ and $F(a) = F(b)$. Let $a = a_1 a_2 \ldots$ and $b = b_1 b_2 \ldots$ where $a$'s representation does not have infinitely repeating $(q-1)$s. There exists some maximal $n$ such that $a_i = b_i$ for $i<n$. Furthermore, let $k$ be minimal such that $k > n$, $a_{k} < q-1$. Define $w$ as the finite prefix $a_1 \ldots a_n \ldots a_{k-1} q-1$, and note that $a < [w] < b$. \mycomment[wms]{There should also be an argument based on the cylinder sets generating the $\sigma$-algebra but I like that this is constructive.} Hence $\mathbb{P}[X^\infty \in [w]] = 0$ as $F(a) = F(b)$. We have that, for some $j$ appearing in $w$, $\mathbb{P}(X^\infty \in [j]) = 0$ and consequently $p_j = 0$. \mycomment[wms]{Separately, we could argue a relationship between the shift operator and $F$ (as we were discussing in the meeting), but I think it is not necessary. The relationship is also not as clear as when $p=1/q$.}
%\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ~~~~~ Stuff that was in the main tex file, but commented out. ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%

The following is a thorough proof of the recursion formula given in (\ref{qsideddierecursion}) for $q=3$, where each case is considered in detail.  Given $x\in [0,1]$, we have 3 cases: $x\in [0, \textstyle \frac{1}{3}]$, $x\in [\textstyle \frac{1}{3}, \frac{2}{3}]$, and $x\in [\textstyle \frac{2}{3},1]$. In any case, we are investigating $F(x) = \mathbb{P}[X_\infty\leq x]$, where $x_i\in \{0,1,2\}$ denotes the ternary expansion for $X_\infty = \sum_{i=1}^\infty \frac{x_i}{3^i}$.

In the case that $x\in [0, \textstyle \frac{1}{3}]$, the \textit{first} ternary interval of rank 1. Thus, $X_\infty \leq x$ can only occur if $x_1=0$.  In this case, we see that
\begin{align*}
    F(x) = \mathbb{P}[X_{\infty} \leq x] &= \mathbb{P}\left[x_1=0 \ \text{and} \ \sum_{i=2}^\infty \frac{x_i}{3^i} \leq x\right]\\ 
    &= p_0\mathbb{P}\left[\sum_{i=2}^\infty \frac{x_i}{3^{i-1}} \leq 3x\right]\\
    &= p_0 \mathbb{P}\left[\sum_{i=1}^\infty \frac{x_{i+1}}{3^{i}} \leq 3x\right]\\
    &= p_0 \mathbb{P}\left[X_\infty \leq 3x\right]\\
    &= p_0 F(3x).
\end{align*}
Of importance is that, when $x\in [0, \textstyle \frac{1}{3}]$, we have that $3x \in [0,1] = \text{dom}(F)$, so that the recursion is well-defined.  

In the case that $x\in [\textstyle \frac{1}{3}, \frac{2}{3}]$, the \textit{second} ternary interval of rank 1. Thus, $X_\infty \leq x$ can occur in two different ways. Specifically
\begin{align*}
    F(x) = \mathbb{P}[X_{\infty} \leq x] &= \mathbb{P}\left[x_1=0 \ \text{or} \ \left(x_1=1 \ \text{and} \ \frac{1}{3} + \sum_{i=2}^\infty \frac{x_i}{3^i} \leq x\right)\right]\\
    &= p_0 + p_1\mathbb{P}\left[1 + \sum_{i=2}^\infty \frac{x_i}{3^{i-1}} \leq 3x\right]\\
    &= p_0 + p_1\mathbb{P}\left[\sum_{i=1}^\infty \frac{x_{i+1}}{3^{i}} \leq 3x-1\right]\\
    &= p_0 + p_1\mathbb{P}\left[X_\infty \leq 3x-1\right]\\
    &= p_0 + p_1F(3x-1).\\
\end{align*}
Similarly, we see that when $x\in [\textstyle \frac{1}{3}, \frac{2}{3}]$, we have that $3x-1 \in [0,1]$.

Finally, we consider $x\in [\textstyle \frac{2}{3},1]$, the \textit{third} ternary interval of rank 1. Here, $X_\infty \leq x$ can occur in three different ways:
\begin{align*}
    F(x) = \mathbb{P}[X_{\infty} \leq x] &= \mathbb{P}\left[x_1=0 \ \text{or} \ x_1=1 \ \text{or} \  \left(x_1=2 \ \text{and} \ \frac{2}{3} + \sum_{i=2}^\infty \frac{x_i}{3^i} \leq x\right)\right]\\
    &= p_0 + p_1 + p_2\mathbb{P}\left[2 + \sum_{i=2}^\infty \frac{x_i}{3^{i-1}} \leq 3x\right]\\
    &= p_0 + p_1 + p_2\mathbb{P}\left[\sum_{i=1}^\infty \frac{x_{i+1}}{3^{i}} \leq 3x-2\right]\\
    &= p_0 + p_1 + p_2\mathbb{P}\left[X_\infty \leq 3x-2\right]\\
    &= p_0 + p_1 + p_2F(3x-2).\\
\end{align*}
Again, we see that when $x\in [\textstyle \frac{2}{3}, 1]$, we have that $3x-2 \in [0,1]$. This suggests how we can extend to the base-$q$ case.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 
 \vspace{1pc}
 
 Of course, all of this works for a $q$-sided die as well. Essentially, (\ref{eq:probarg}) is asking that
 \[
E(\text{random outcome of a fair dice roll}) \neq E(\text{random outcome of the unfair dice roll})
\]
 So here is the question: What can we say about the two hypotheses?
 \begin{enumerate}[(i)]
     \item $p_i\neq \frac{1}{3}$ for all $i$
     \item $p_0\cdot 0 + p_1\cdot 1 + p_2\cdot 2 \neq \frac{1}{3}\cdot 0+\frac{1}{3}\cdot 1+\frac{1}{3}\cdot 2$
 \end{enumerate}
 We see that (ii)$\centernot\implies$(i) by considering $p_0=\textstyle \frac{5}{9}$, $p_1=\textstyle \frac{1}{3}=\frac{3}{9}$, and $p_2=\textstyle \frac{1}{9}$, where (ii) is satisfied, but (i) is not. However, we also see that (i)$\centernot\implies$(ii) by considering $p_0=\textstyle \frac{4}{9}$, $p_1=\textstyle \frac{1}{9}$, and $p_2=\textstyle \frac{4}{9}$, where (i) is satisfied, but (ii) is not.
 
 Thus, our two results conclude that $F$ is singular, but with different hypotheses on the probabilities -- neither of which imply the other. From a certain perspective, the above two hypotheses ask the following:
  \begin{enumerate}[(i)]
     \item Is the die always \textit{locally} unfair?
     \item Is the die \textit{globally} unfair?
 \end{enumerate}
 Where the previous choices of $p_i$ support the notion that one doesn't preclude/imply the other.
 \begin{remark}
 This dichotomy is only relevant when $q\geq 3$. In the coinflip case, when $q=2$, (i) and (ii) are the same.
 \end{remark}
 
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Old proof of $F$'s singularity when all $p_j\neq \frac{1}{q}$:
 
 Additionally, we note that $F'(x)=0$ for $x\notin [0,1]$. One can see this by observing the following. If $x<0$, then $F(x) = \mathbb{P}[X_\infty \leq x]=0$ since $X_\infty\geq0$. If $x>1$, then $F(x) = \mathbb{P}[X_\infty \leq x]=1$ since $X_\infty \leq 1$. Therefore $F$ is constant outside of $[0,1]$, meaning $F'(x)=0$.

Now, suppose that $0<x<1$ so that $F'(x)$ exists. We show that $F'(x)=0$. To this end, for each $n$, choose $k_n$ so that $x \in I_n$, where
\[
I_n = \left( \frac{k_n}{q^n}, \frac{k_n+1}{q^n}\right)
\]
is the base-$q$ interval of rank $n$ that contains $x$. Along with the density of the base-$q$ numbers in $[0,1]$, it follows from (\ref{interval1}) and (\ref{interval2}) above that
\begin{equation}
    \lim_{n\to\infty} \frac{ \mathbb{P}[X_\infty \in I_n]}{q^n} = \lim_{n\to\infty} \frac{ F\left( \frac{k+1}{q^n}\right) - F\left( \frac{k}{q^n}\right)   }{q^n} = F'(x).
\end{equation}
Therefore, if we suppose, for the sake of contradiction, that $F'(x)\neq 0$, then on one hand we obtain the following:
\begin{equation}
    \lim_{n\to\infty} \frac{\frac{ \mathbb{P}[X_\infty \in I_{n+1}]}{q^{n+1}}}{ \frac{ \mathbb{P}[X_\infty \in I_{n}]}{q^n} } = \frac{F'(x)}{F'(x)}=1.
\end{equation}
Thus, 
\begin{equation} \label{1/qcont}
    \lim_{n\to\infty} \frac{ \mathbb{P}[X_\infty \in I_{n+1}]}{ \mathbb{P}[X_\infty \in I_{n}] } = \frac{1}{q}.
\end{equation}
On the other hand, We know that $I_n$ consists of those numbers in $[0,1]$ whose base-$q$ expansions match $x$'s for the first $n$ terms. Thus, if $X_\infty \in I_n$, then 
\[
X_\infty = \sum_{i=1}^n \frac{u_i}{q^i} + \sum_{i=n+1}^\infty \frac{x_i}{q^i}.
\]
This implies that $\mathbb{P}[X_\infty \in I_n] = p_{u_1}\cdot p_{u_2}\cdot\ldots \cdot p_{u_n}$. Therefore,
\begin{equation}
    \frac{ \mathbb{P}[X_\infty \in I_{n+1}]}{ \mathbb{P}[X_\infty \in I_{n}] } = \frac{  p_{u_1}\cdot p_{u_2}\cdot\ldots \cdot p_{u_n} \cdot p_{u_{n+1}}}{p_{u_1}\cdot p_{u_2}\cdot\ldots \cdot p_{u_n}} = p_{ u_{n+1} } \neq \frac{1}{q}.
\end{equation}
\textcolor{blue}{To contradict (\ref{1/qcont}), we need only show that $\displaystyle\lim_{n\to\infty}p_{u_{n+1}} \neq \frac{1}{q}$. But what is this limit? It is a limit of probabilities for the $n+1^{\text{th}}$ roll of the die. That is, the sequence $(p_{u_{n+1}})$ is taken from the finite set $\{p_0,p_1,\ldots,p_{q-1}\}$. This implies that the sequence has a convergent subsequence (in fact, a constant subsequence), but it does not necessarily imply overall convergence. For this to occur, you need a tail to be always equal to the limit value. In this case, this means there exists an $N$ such that $p_{u_{n+1}} = \frac{1}{q}$ for all $n+1\geq N$. The only way this happens is if our \textit{arbitrary} sequence of outcomes $(u_1,u_2,\ldots)$ began returning the same subcollection of outcomes from some point onward. This is unreasonable\mycomment[DTP]{Is there a more rigorous way to assert this?} unless we are in the situation that \textit{every} outcome has probability $\frac{1}{q}$ -- but then this is the fair case that we are explicitly avoiding. Thus, it is not possible for this limit to exist -- THAT is the contradiction to line (\ref{1/qcont}).}
\textcolor{red}{As Darby noted, this reasoning is incorrect, since all sequences must be accounted for. We try another approach via arclength later.}

This contradicts the conclusion yielded in (\ref{1/qcont}). Thus, $F'(x) = 0$ almost everywhere and therefore $F$ is singular.

%We organize this effort as follows. In Section \ref{sec:bernoulli}, we define binary encoded distributions from Bernoulli coinflips and summarize existing results. Then, we establish the main results regarding the CFD of the $q$-sided die and deviations from uniform in Section~\ref{sec:qsideddie}. Section~\ref{sec:arclength} provides an arclength analysis for a finite number of ``dice rolls.''  Lastly, we provide some concluding remarks in Section~\ref{sec:conclusion}.\mycomment[jds]{Revisit this structure paragraph once we are done with the polish.}

%\begin{exmp}
%One can verify directly that, in base 10,
%\[
%0.8125 = \frac{1}{2^1} + \frac{1}{2^2} + \frac{0}{2^3} + \frac{1}{2^4}
%\]
%and so $0.8125_{10} = 0.1101_2$.
%\end{exmp}

%https://web.maths.unsw.edu.au/%7Ejosefdick/preprints/KuipersNied_book.pdf


%Consider a $q$-sided die, where $x_i\in\{0,\ldots,q-1\}$ denotes the outcome of the $i^\text{th}$ toss and $p_j:=\mathbb{P}[x_i=j]$ for $j\in\{0,\ldots,q-1\}$. Given $X = \sum_{i=1}^\infty x_iq^{-i}$, let $F(x)=\mathbb{P}[X\leq x]$ be the cumulative distribution function obtained after tossing the die an infinite number of times. Let $P^n =\{v_i\}_{i=1}^{q^n}$ be the set of $q$-tuples described in the conversation preceding Remark \ref{remark:tags}. 

%Imagine then, if one had a chip full of coin-like devices all weighted to a particular probability $p$ of heads.  If one had access to the probability measure induced by each device and had access to the set of all binary numbers with density $p$ of 1's, then one could evaluate the measure of each device on this set.  If the measure returns 1, then the device is weighted correctly, otherwise the device would return zero.  This would provide an immediate indicator that the chip was manufactured or tuned correctly.  Obviously, having such a distributional object on hand is in the realm of fantasy.  Nonetheless, having this theory touchpoint that provides so clear of a test of weighting is an excellent starting point to finding validation measures and metrics for real devices.
